Social Learning: Towards Collaborative Learning with Large Language Models

We introduce the framework of "social learning" in the context of large language models (LLMs), whereby models share knowledge with each other in a privacy-aware manner using natural language. We present and evaluate two approaches for knowledge transfer between LLMs. In the first scenario, we allow the model to generate abstract prompts aiming to teach the task. In our second approach, models transfer knowledge by generating synthetic examples. We evaluate these methods across diverse datasets and quantify memorization as a proxy for privacy loss. These techniques inspired by social learning yield promising results with low memorization of the original data. In particular, we show that performance using these methods is comparable to results with the use of original labels and prompts. Our work demonstrates the viability of social learning for LLMs, establishes baseline approaches and highlights several unexplored areas for future work.

==> original_p_values_without_half.tex <==
\begin{table*}[t]
    \centering
    \begin{minipage}{.9\linewidth}
    \renewcommand\footnoterule{}
    %\centering
    \begin{tabular}{c|c|c|c|c|c|c|c}\toprule
    $n$ & Type & Lambada & BoolQ  & GSM8K & SMS Spam & \parbox[t]{60pt}{\centering SMS Spam\\(With Class)} & \parbox[t]{60pt}{\centering Random\\Insertion}\\\midrule
    0 & -   &  69.80(0.00) &  68.10(0.00) &   0.00(0.00)\footnote{GSM8K uses a special format to mark the answer. The model inevitably always fails when no instruction or examples are provided to it to clarify this special format. Adding the prefix stated in Figure~\ref{fig:gsm8k_prefix} to clarify the format yields accuracy 16.38\%. } &  14.19(0.00) &  92.70(0.00) &  22.00(0.00) \\
    \midrule
\multirow{3}{*}{1} & Private &  86.68(0.48) &  89.84(0.10) &  63.59(0.25) &  59.10(7.62) &  94.25(0.27) &  55.56(3.12) \\
& Artificial &  86.65(0.44) &  70.46(7.19) &  63.87(0.76) &  90.22(0.57) &  92.55(0.40) &  53.58(7.89) \\
& {\small $p$-value}                 &  {\small 0.9790} &  {\small 0.0000} &  {\small 0.7415} &  {\small 0.0000} &  {\small 0.0046} &  {\small 0.0471} \\
%& \makecell{Artificial\\{\small$p$-value}}  &  \makecell{86.65(0.44)\\{\small0.9790}} &  \makecell{70.46(7.19)\\{\small0.0000}} &  \makecell{63.87(0.76)\\{\small0.7415}} &  \makecell{90.22(0.57)\\{\small0.0000}} &  \makecell{92.55(0.40)\\{\small0.0046}} &  \makecell{53.58(7.89)\\{\small0.0471}} \\
\midrule

\multirow{3}{*}{2} & Private   &  87.30(0.44) &  90.12(0.03) &  64.20(0.28) &  77.15(9.96) &  94.87(0.25) &  70.04(3.19) \\
& Artificial                 &  86.70(0.41) &  88.63(0.77) &  63.23(0.60) &  88.17(0.74) &  92.15(0.63) &  65.94(1.75) \\
& {\small $p$-value}               &  {\small 0.4137} &  {\small 0.0000} &  {\small 0.2534} &  {\small 0.0000} &  {\small 0.0000} &  {\small 0.0000} \\
%& \makecell{Artificial\\{\small$p$-value}}   &  \makecell{86.70(0.41)\\{\small0.4137}} &  \makecell{88.63(0.77)\\{\small0.0000}} &  \makecell{63.23(0.60)\\{\small0.2534}} &  \makecell{88.17(0.74)\\{\small0.0000}} &  \makecell{92.15(0.63)\\{\small0.0000}} &  \makecell{65.94(1.75)\\{\small0.0000}} \\
\midrule

\multirow{3}{*}{4} & Private  &  87.56(0.63) &  90.44(0.07) &  63.59(0.27) &  86.75(8.28) &  95.43(0.53) &  69.74(2.55) \\
&Artificial                              &  87.98(0.43) &  85.54(3.87) &  63.58(0.48) &  87.77(0.75) &  90.19(0.81) &  69.72(2.42) \\
&{\small $p$-value}                   &  {\small 0.5619} &  {\small 0.0000} &  {\small 1.0000} &  {\small 0.1981} &  {\small 0.0000} &  {\small 1.0000} \\
%& \makecell{Artificial\\{\small$p$-value}}   &  \makecell{87.98(0.43)\\{\small0.5619}} &  \makecell{85.54(3.87)\\{\small0.0000}} &  \makecell{63.58(0.48)\\{\small1.0000}} &  \makecell{87.77(0.75)\\{\small0.1981}} &  \makecell{90.19(0.81)\\{\small0.0000}} &  \makecell{69.72(2.42)\\{\small1.0000}} \\
\midrule

\multirow{3}{*}{8} & Private   &  88.36(0.54) &  90.53(0.07) &  64.05(0.23) &  96.02(0.27) &  96.75(0.11) &  74.50(1.15) \\
&Artificial                             &  88.05(0.27) &  88.73(0.88) &  63.38(0.47) &  86.45(0.88) &  91.51(0.97) &  69.22(3.42) \\
&{\small $p$-value}                  &  {\small 0.6493} &  {\small 0.0000} &  {\small 0.4328} &  {\small 0.0000} &  {\small 0.0000} &  {\small 0.0000} \\
%& \makecell{Artificial\\{\small$p$-value}}   &   \makecell{88.05(0.27)\\{\small0.6493}} &  \makecell{88.73(0.88)\\{\small0.0000}} &  \makecell{63.38(0.47)\\{\small0.4328}} &  \makecell{86.45(0.88)\\{\small0.0000}} &  \makecell{91.51(0.97)\\{\small0.0000}} &  \makecell{69.22(3.42)\\{\small0.0000}} \\
\midrule

\multirow{3}{*}{16} & Private &  88.40(0.67) &  90.42(0.08) &  63.55(0.28) &  96.48(0.17) &  97.02(0.07) &  73.52(1.11) \\
&Artificial                             &  89.04(0.23) &  89.94(0.08) &  63.71(0.35) &  87.98(1.18) &  91.08(1.57) &  72.36(1.01) \\
&{\small $p$-value}                  &  {\small 0.3495} &  {\small 0.1512} &  {\small 0.8532} &  {\small 0.0000} &  {\small 0.0000} &  {\small 0.2046} \\
%& \makecell{Artificial\\{\small$p$-value}}  &  \makecell{89.04(0.23)\\{\small0.3495}} &  \makecell{89.94(0.08)\\{\small0.1512}} &  \makecell{63.71(0.35)\\{\small0.8532}} &  \makecell{87.98(1.18)\\{\small0.0000}} &  \makecell{91.08(1.57)\\{\small0.0000}} &  \makecell{72.36(1.01)\\{\small0.2046}} \\
\bottomrule
    \end{tabular}
    \end{minipage}
    \caption{This table reports accuracies and $p$-values reported in Table~\ref{tab:artificial-examples-results-same-size} with more precision.}
    \label{tab:artificial-examples-results-same-size-detailed}
\end{table*}

\begin{table*}[t]
    \centering
    \begin{minipage}{\linewidth}
    \renewcommand\footnoterule{}
    \centering
    \begin{tabular}{c|c|c|c|c|c|c|c|c}\toprule
    $n$ & Type & Student & Lambada & BoolQ  & GSM8K & SMS Spam & \parbox[t]{60pt}{\centering SMS Spam\\(With Class)} & \parbox[t]{60pt}{\centering Random\\Insertion}\\\midrule
    \multirow{4}{*}{1} & Private & PaLM 2-XS  &  74.61(2.15) &  81.05(1.02) &   9.28(2.04) &  61.75(4.55) &  54.30(1.88) &  11.80(3.37) \\
& Private & PaLM 2-S                           &  86.68(0.48) &  89.84(0.10) &  63.59(0.25) &  59.10(7.62) &  94.25(0.27) &  55.56(3.12) \\
&\small{\makecell{Artificial\\ PaLM2-XS}}       & PaLM 2-S                         &      86.72(0.72) &      72.17(6.46) &      57.21(4.83) &      75.94(7.89) &      92.42(1.51) &      50.92(3.25) \\
&\multicolumn{2}{c|}{\small $p$-value}     &  {\small 0.9766} &  {\small 0.0000} &  {\small 0.0000} &  {\small 0.0000} &  {\small 0.0024} &  {\small 0.0000} \\
%& \makecell{\small{Artificial PaLM2-XS}\\{\small$p$-value}} & PaLM 2-S                       &   \makecell{86.72(0.72)\\{\small0.9766}} &  \makecell{72.17(6.46)\\{\small0.0000}} &  \makecell{57.21(4.83)\\{\small0.0000}} &  \makecell{75.94(7.89)\\{\small0.0000}} &  \makecell{92.42(1.51)\\{\small0.0024}} &  \makecell{50.92(3.25)\\{\small0.0000}} \\
\midrule

\multirow{4}{*}{2} & Private & PaLM 2-XS  &  73.65(3.22) &  80.94(0.98) &  16.03(0.26) &  72.15(8.16) &  75.11(9.25) &  19.94(2.60) \\
& Private & PaLM 2-S                         &  87.30(0.44) &  90.12(0.03) &  64.20(0.28) &  77.15(9.96) &  94.87(0.25) &  70.04(3.19) \\
&\small{\makecell{Artificial\\ PaLM2-XS}}    & PaLM 2-S                            &      87.84(0.53) &      89.75(0.15) &      63.55(0.58) &      59.73(6.78) &      87.88(3.55) &      66.10(1.25) \\
&\multicolumn{2}{c|}{\small $p$-value}     &  {\small 0.4479} &  {\small 0.2692} &  {\small 0.4422} &  {\small 0.0000} &  {\small 0.0000} &  {\small 0.0000} \\
%& \makecell{\small{Artificial PaLM2-XS}\\{\small$p$-value}} & PaLM 2-S                     & \makecell{87.84(0.53)\\{\small0.4479}} &  \makecell{89.75(0.15)\\{\small0.2692}} &  \makecell{63.55(0.58)\\{\small0.4422}} &  \makecell{59.73(6.78)\\{\small0.0000}} &  \makecell{87.88(3.55)\\{\small0.0000}} &  \makecell{66.10(1.25)\\{\small0.0000}} \\
\midrule

\multirow{4}{*}{4} & Private & PaLM 2-XS  &  81.48(2.90) &  81.11(0.22) &  19.15(0.65) &  90.43(1.41) &  94.92(0.66) &  25.14(1.94) \\
& Private & PaLM 2-S                         &  87.56(0.63) &  90.44(0.07) &  63.59(0.27) &  86.75(8.28) &  95.43(0.53) &  69.74(2.55) \\
&\small{\makecell{Artificial\\ PaLM2-XS}}     & PaLM 2-S                           &      88.05(0.26) &      82.82(4.48) &      63.85(0.64) &      94.09(0.44) &      93.87(0.51) &      51.46(0.43) \\
&\multicolumn{2}{c|}{\small $p$-value}      &  {\small 0.4744} &  {\small 0.0000} &  {\small 0.7693} &  {\small 0.0000} &  {\small 0.0038} &  {\small 0.0000} \\
% & \makecell{\small{Artificial PaLM2-XS}\\{\small$p$-value}} & PaLM 2-S                     &    \makecell{88.05(0.26)\\{\small0.4744}} &  \makecell{82.82(4.48)\\{\small0.0000}} &  \makecell{63.85(0.64)\\{\small0.7693}} &  \makecell{94.09(0.44)\\{\small0.0000}} &  \makecell{93.87(0.51)\\{\small0.0038}} &  \makecell{51.46(0.43)\\{\small0.0000}} \\
\midrule

\multirow{4}{*}{8} & Private & PaLM 2-XS  &  86.20(0.43) &  81.90(0.27) &  18.61(0.44) &  95.73(0.59) &  96.45(0.23) &  31.44(2.43) \\
& Private & PaLM 2-S                         &  88.36(0.54) &  90.53(0.07) &  64.05(0.23) &  96.02(0.27) &  96.75(0.11) &  74.50(1.15) \\
&\small{\makecell{Artificial\\ PaLM2-XS}}       & PaLM 2-S                          &      89.12(0.11) &      90.18(0.08) &      62.64(0.77) &      94.62(0.29) &      96.13(0.30) &      63.26(2.46) \\
&\multicolumn{2}{c|}{\small $p$-value}     &  {\small 0.2527} &  {\small 0.3022} &  {\small 0.0994} &  {\small 0.0057} &  {\small 0.1688} &  {\small 0.0000} \\
%& \makecell{\small{Artificial PaLM2-XS}\\{\small$p$-value}} & PaLM 2-S                     &  \makecell{89.12(0.11)\\{\small0.2527}} &  \makecell{90.18(0.08)\\{\small0.3022}} &  \makecell{62.64(0.77)\\{\small0.0994}} &  \makecell{94.62(0.29)\\{\small0.0057}} &  \makecell{96.13(0.30)\\{\small0.1688}} &  \makecell{63.26(2.46)\\{\small0.0000}} \\
\midrule

\multirow{4}{*}{16} & Private & PaLM 2-XS &  87.26(0.24) &  82.62(0.35) &  17.68(0.45) &  96.34(0.35) &  96.16(0.39) &  30.22(1.70) \\
 & Private & PaLM 2-S                          &  88.40(0.67) &  90.42(0.08) &  63.55(0.28) &  96.48(0.17) &  97.02(0.07) &  73.52(1.11) \\
 &\small{\makecell{Artificial\\ PaLM2-XS}}      & PaLM 2-S                           &      89.18(0.33) &      89.08(0.99) &      63.75(0.71) &      94.62(0.47) &      93.95(1.11) &      61.76(3.49) \\
&\multicolumn{2}{c|}{\small $p$-value}         &  {\small 0.2392} &  {\small 0.0000} &  {\small 0.8240} &  {\small 0.0004} &  {\small 0.0000} &  {\small 0.0000} \\
 %& \makecell{\small{Artificial PaLM2-XS}\\{\small$p$-value}} & PaLM 2-S                      & \makecell{89.18(0.33)\\{\small0.2392}} &  \makecell{89.08(0.99)\\{\small0.0000}} &  \makecell{63.75(0.71)\\{\small0.8240}} &  \makecell{94.62(0.47)\\{\small0.0004}} &  \makecell{93.95(1.11)\\{\small0.0000}} &  \makecell{61.76(3.49)\\{\small0.0000}} \\
 
\bottomrule
    \end{tabular}
    \end{minipage}
    \caption{This table reports accuracies and $p$-values reported in Table~\ref{tab:artificial-examples-results-small-teachers} with more precision.}
    \label{tab:artificial-examples-results-small-teachers-detailed}
\end{table*}


\begin{table*}[t]
    \centering
    
    
    \begin{tabular}{c|c|c|c|c|c|c|c}\toprule
    $n$&Method & Lambada & BoolQ  & GSM8K & SMS Spam & \parbox[t]{60pt}{\centering SMS Spam\\(With Class)} & \parbox[t]{60pt}{\centering Random\\Insertion}\\\midrule
    
    \multirow{3}{*}{1}&\makecell{Random}                                                               &       86.65(0.44) &  70.46(7.19) &                          63.87(0.76) &                          90.22(0.57) &                         92.55(0.40) &                          53.58(7.89) \\
    &Voting                       &      86.50(0.28) &      86.63(2.60) &      60.52(1.07) &      87.31(0.61) &      93.15(0.24) &      56.56(3.66) \\
&{\small $p$-value}           &  {\small 0.6244} &  {\small 0.0000} &  {\small 0.0000} &  {\small 0.0001} &  {\small 0.3423} &  {\small 0.0039} \\
   % &\makecell{Voting \\ {\small $p$-value}}                                                          &                          \makecell{86.50(0.28)\\{\small 0.6244}} &                          \makecell{86.63(2.60)\\{\small 0.0000}} &                          \makecell{60.52(1.07)\\{\small 0.0000}} &                          \makecell{87.31(0.61)\\{\small 0.0001}} &                          \makecell{93.15(0.24)\\{\small 0.3423}} &                          \makecell{56.56(3.66)\\{\small 0.0039}} \\
    \midrule
    
    \multirow{3}{*}{2}&\makecell{Random}                                                               &                          86.70(0.41) &                          88.63(0.77) &                          63.23(0.60) &                          88.17(0.74) &                          92.15(0.63) &                         65.94(1.75) \\
    &Voting                       &      87.87(0.28) &      85.80(2.81) &      64.75(0.33) &      83.74(2.19) &      88.06(1.71) &      67.84(1.29) \\
&{\small $p$-value}           &  {\small 0.0002} &  {\small 0.0000} &  {\small 0.0734} &  {\small 0.0000} &  {\small 0.0000} &  {\small 0.0457} \\
    %&\makecell{Voting \\ {\small $p$-value}}                                                          &                          \makecell{87.87(0.28)\\{\small 0.0002}} &                          \makecell{85.80(2.81)\\{\small 0.0000}} &                          \makecell{64.75(0.33)\\{\small 0.0734}} &                          \makecell{83.74(2.19)\\{\small 0.0000}} &                          \makecell{88.06(1.71)\\{\small 0.0000}} &                          \makecell{67.84(1.29)\\{\small 0.0457}} \\
    \midrule
    
    \multirow{3}{*}{4}&\makecell{Random}                                                              &                          87.98(0.43) &                          85.54(3.87) &                          63.58(0.48) &                          87.77(0.75) &                          90.19(0.81) &                          69.72(2.42) \\
     &Voting                        &      88.18(0.33) &      89.76(0.22) &      64.82(0.42) &      84.11(1.94) &      91.05(0.96) &      72.90(2.07) \\
&{\small $p$-value }           &  {\small 0.4816} &  {\small 0.0000} &  {\small 0.1382} &  {\small 0.0000} &  {\small 0.2254} &  {\small 0.0002} \\
    %&\makecell{Voting \\ {\small $p$-value}}                                                          &                          \makecell{88.18(0.33)\\{\small 0.4816}} &                          \makecell{89.76(0.22)\\{\small 0.0000}} &                          \makecell{64.82(0.42)\\{\small 0.1382}} &                          \makecell{84.11(1.94)\\{\small 0.0000}} &                          \makecell{91.05(0.96)\\{\small 0.2254}} &                          \makecell{72.90(2.07)\\{\small 0.0002}} \\
    \midrule
    
    \multirow{3}{*}{8}&\makecell{Random}                                                               &                         88.05(0.27) &                          88.73(0.88) &                          63.38(0.47) &                          86.45(0.88) &                          91.51(0.97) &                          69.22(3.42)\\
     &Voting                        &      88.22(0.20) &      89.53(0.30) &      64.03(0.32) &      84.78(1.96) &      89.52(1.12) &      71.36(0.98) \\
&{\small $p$-value }           &  {\small 0.5618} &  {\small 0.0185} &  {\small 0.4432} &  {\small 0.0460} &  {\small 0.0038} &  {\small 0.0197} \\
    %&\makecell{Voting \\ {\small $p$-value}}                                                          &                          \makecell{88.22(0.20)\\{\small 0.5618}} &                          \makecell{89.53(0.30)\\{\small 0.0185}} &                          \makecell{64.03(0.32)\\{\small 0.4432}} &                          \makecell{84.78(1.96)\\{\small 0.0460}} &                          \makecell{89.52(1.12)\\{\small 0.0038}} &                          \makecell{71.36(0.98)\\{\small 0.0197}} \\
    \midrule
    
    \multirow{3}{*}{16}&\makecell{Random}                                                               &                          89.04(0.23) &                          89.94(0.08) &                          63.71(0.35) &                          87.98(1.18) &                          91.08(1.57) &                          72.36(1.01) \\
 &Voting                       &      88.76(0.25) &      89.65(0.09) &      63.53(0.36) &      87.85(3.04) &      89.44(1.26) &      72.82(2.18) \\
&{\small $p$-value }           &  {\small 0.3226} &  {\small 0.3911} &  {\small 0.8391} &  {\small 0.8854} &  {\small 0.0179} &  {\small 0.6233} \\
%&\makecell{Voting \\ {\small $p$-value}}                                                         &                          \makecell{88.76(0.25)\\{\small 0.3226}} &                          \makecell{89.65(0.09)\\{\small 0.3911}} &                          \makecell{63.53(0.36)\\{\small 0.8391}} &                          \makecell{87.85(3.04)\\{\small 0.8854}} &                          \makecell{89.44(1.26)\\{\small 0.0179}} &                          \makecell{72.82(2.18)\\{\small 0.6233}} \\
    \bottomrule
    \end{tabular}
    \caption{This table reports accuracies and $p$-values reported in Table~\ref{tab:aggregation-results} with more precision.}
    \label{tab:aggregation-results-detailed}
\end{table*}

\begin{table*}[t]
    \centering
    \begin{minipage}{\linewidth}
    \renewcommand\footnoterule{}
    \centering
    \begin{tabular}{c|c|c|c|c|c|c}\toprule
    Method & Lambada & BoolQ  & GSM8K & SMS Spam & \parbox[t]{60pt}{\centering SMS Spam\\(With Class)} & \parbox[t]{60pt}{\centering Random\\Insertion}\\\midrule
    Zero-Shot &  69.80 &  68.10 &   0.00
    %\footnote{\label{tab:instruction-examples:footnote_gsm8k}The model inevitably always fails when no instruction or examples are provided to it to clarify the special format of GSM8K. Cells marked with (\ref{tab:instruction-examples:footnote_gsm8k}) report the accuracy with the prefix stated in Figure~\ref{fig:gsm8k_prefix} manually added to clarify the format instead of reporting the trivial 0.00 accuracy. } 
    &  14.19 &  92.70 &  22.00 \\
 Manual           &  77.45 &  90.18 &  15.62 &  93.95 &  94.22 &  34.9 \\
 \midrule
 8-shot Private Examples   &  88.36(0.54) &  90.53(0.07) &  64.05(0.23) &  96.02(0.27) &  96.75(0.11) &  74.50(1.15) \\
8-shot Artificial Examples   &  88.05(0.27) &  88.73(0.88) &  63.38(0.47) &  86.45(0.88) &  91.51(0.97) &  69.22(3.42) \\
\midrule
%\parbox{.2\textwidth}{\centering Generated Instruction (GPT3.5)\vspace{-5pt}\\{\scriptsize $p$-value (8-shot private)}\vspace{-5pt}\\{\scriptsize $p$-value (zero-shot)}}        &       \makecell{80.87\vspace{-5pt}\\{\scriptsize0.0000}\vspace{-5pt}\\{\scriptsize0.0000}} &      \makecell{90.06\vspace{-5pt}\\{\scriptsize0.4109}\vspace{-5pt}\\{\scriptsize0.0000}} &      \makecell{11.30\vspace{-5pt}\\{\scriptsize0.0000}\vspace{-5pt}\\{\scriptsize0.0000}} &      \makecell{93.82\vspace{-5pt}\\{\scriptsize0.0076}\vspace{-5pt}\\{\scriptsize0.0000}} &      \makecell{93.95\vspace{-5pt}\\{\scriptsize0.0002}\vspace{-5pt}\\{\scriptsize0.3575}} &      \makecell{43.80\vspace{-5pt}\\{\scriptsize0.0000}\vspace{-5pt}\\{\scriptsize0.0000}} \\
GPT3.5 Generated Inst.                                                            &                                                                             82.81(1.87) &                                                                             90.12(0.07) &                                                                              4.11(2.27) &                                                                             85.38(8.70) &                                                                             95.38(0.37) &                                                                             59.22(4.76) \\


PaLM 2-S Generated Inst.                                                                                         &                                                                             85.12(0.91) &                                                                             88.74(1.36) &                                                                              0.00(0.00) &                                                                             92.90(0.04) &                                                                             93.44(0.39) &                                                                             40.38(9.88) \\



%\makecell{Gen. Inst. (340B)\vspace{-5pt}\\{\scriptsize $p$-value (8-shot private)}\vspace{-5pt}\\{\scriptsize $p$-value (zero-shot)}}        &    \makecell{83.47\vspace{-5pt}\\{\scriptsize0.0000}\vspace{-5pt}\\{\scriptsize0.0000}} &      \makecell{88.53\vspace{-5pt}\\{\scriptsize0.0006}\vspace{-5pt}\\{\scriptsize0.0000}} &       \makecell{15.60\footnoteref{tab:instruction-examples:footnote_gsm8k}\vspace{-5pt}\\{\scriptsize0.0000}\vspace{-5pt}\\{\scriptsize0.0000}} &      \makecell{85.22\vspace{-5pt}\\{\scriptsize0.0000}\vspace{-5pt}\\{\scriptsize0.0000}} &      \makecell{90.86\vspace{-5pt}\\{\scriptsize0.0000}\vspace{-5pt}\\{\scriptsize0.2271}} &       \makecell{0.60\vspace{-5pt}\\{\scriptsize0.0000}\vspace{-5pt}\\{\scriptsize0.0000}} \\

         \bottomrule
    \end{tabular}
    \end{minipage}
    \caption{This table reports accuracies and $p$-values reported in Table~\ref{tab:instruction-results} with more precision.}
    \label{tab:instruction-results-detailed}
\end{table*}
